CryptoMask : Privacy-preserving Face Recognition

Face recognition is a widely-used technique for identification or verification, where a verifier checks whether a face image matches anyone stored in a database. However, in scenarios where the database is held by a third party, such as a cloud server, both parties are concerned about data privacy. To address this concern, we propose CryptoMask, a privacy-preserving face recognition system that employs homomorphic encryption (HE) and secure multi-party computation (MPC). We design a new encoding strategy that leverages HE properties to reduce communication costs and enable efficient similarity checks between face images, without expensive homomorphic rotation. Additionally, CryptoMask leaks less information than existing state-of-the-art approaches. CryptoMask only reveals whether there is an image matching the query or not, whereas existing approaches additionally leak sensitive intermediate distance information. We conduct extensive experiments that demonstrate CryptoMask's superior performance in terms of computation and communication. For a database with 100 million 512-dimensional face vectors, CryptoMask offers ${\thicksim}5 \times$ and ${\thicksim}144 \times$ speed-ups in terms of computation and communication, respectively.

==> include/relatedwork.tex <==
%shao hang%

\section{Related Work} \label{sec:relatedwork}
For the protection methods of biometric security authentication in the past, we can roughly divide them into protection based on traditional cryptographic algorithms, protection based on pattern recognition and protection based on privacy computing:\par
    
\textbf{Protection based on traditional cryptographic algorithm.} In 1998, Soutar et al. ~\cite{soutar1998biometric}first proposed to apply encryption technology to fingerprint authentication. For example, visual password ~\cite{naor1994visual} can be applied to biometric authentication such as fingerprint identification ~\cite{rao2008fingerprint}, iris identification ~\cite{revenkar2010secure} and face recognition ~\cite{ross2010visual}. In addition, fuzzy value ~\cite{juels2006fuzzy} technology is used to achieve fingerprint authentication ~\cite{uludag2005fuzzy} and iris authentication ~\cite{lee2008new}. Although this method can achieve biometric authentication, However, biometric data may be exposed during authentication and matching, and the matching accuracy is not high.

\textbf{Protection based on pattern recognition.} Unlike the security provided by the encryption algorithm, biometric authentication based on pattern recognition is another security authentication method. For example, Davida et al. ~\cite{davida1998enabling} and Radha et al. ~\cite{ratha2001enhancing} use non invertible transformation functions to protect biometrics. Patel et al. ~\cite{patel2015cancelable} and Jin et al. ~\cite{jin2017ranking} propose a security authentication model of revocability and diversity of templates, This method requires a trade-off between security and matching performance, and is not practical.  
        
\textbf{Protection based on privacy computing.} Shai et al. ~\cite{avidan2006efficient} used encryption in secure multi-party computing to protect features, but the computing speed was slow, and then introduced machine learning to speed up computing efficiency; Shashank et al. ~\cite{shashank2008private} realized image retrieval using the technology of oblivious transfer (OT); Maneesh et al. ~\cite{upmanyu2009efficient} implemented a video surveillance system based on the secret sharing technology constituted by the Chinese Residual Theorem (CRT), which can effectively detect and track personnel; Andy et al. ~\cite{abadi2016deep} used differential privacy to infer and learn privacy data, and then applied it to face recognition systems. Homomorphic encryption can directly calculate the distance of feature vectors (Euclidean distance or cosine distance) in the encryption domain because it can calculate ciphertext directly, and then complete feature matching. Most of the original schemes use partial homomorphic encryption (PHE). For example, Maneesh et al. ~\cite{upmanyu2009efficient2} proposed a biometric matching scheme using the additive homomorphism of Pailllier algorithm, which requires repeated interaction between the client and the data end to calculate the similarity, Therefore, the communication and computing costs are large. By using fully homomorphic encryption(FHE) technology, arbitrary computation can be completely performed between ciphertext, which can effectively reduce the traffic. Troncoso et al. ~\cite{troncoso2013fully} designed a face recognition system based on the early STOC09 ~\cite{gentry2011implementing} fully homomorphic encryption scheme, but its efficiency is low due to the expensive homomorphic computation; In 2018, Vishnu et al. ~\cite{boddeti2018secure} designed a face recognition protection scheme, in which the fully homomorphism encryption of the BFV scheme was used to calculate the cosine distance, and the batch processing (SIMD technology) and dimension reduction technology were used to improve the computing efficiency. For 512 dimensional facial features, it only took 16KB of storage space for each encrypted feature and 0.02s of time to match a pair of encrypted features. In 2022, they proposed a new face recognition framework HERS ~\cite{engelsma2022hers} on the basis of ~\cite{boddeti2018secure}, which optimized the batch processing technology to achieve 1: m matching. Compared with using ciphertext rotation to calculate the inner product, it improved the calculation efficiency. The matching time in 1 million encrypted images was 10 minutes, and the loss of accuracy was controlled within $2\%$. It can be seen that homomorphic encryption is a feasible and practical solution for accurate face matching in the encryption domain, which not only protects user privacy, but also prevents information leakage.  

On the basis of ~\cite{boddeti2018secure} and ~\cite{engelsma2022hers}, our protocol uses a more efficient method to calculate the inner product, and proposes a new encoding method, which compresses data when encoding, further reducing communication and improving computing efficiency. Experiments show that the protocol has better performance and is more suitable for scalable databases\notesh{It can supplement the experimental results}.

==> include/security.tex <==
\section{Complexity and Security Analysis}\label{sec:security}
In this section, we first provide a theoretical complexity analysis to show that CryptoMask can support database with millions records.
% which is extremely expensive in most recent literatures. 
Then we analyze that our face recognition protocol is secure against a semi-honest adversary under the assumption supposing the KG is fully trusted.

\subsection{Complexity Analysis}
In CryptoMask, the communication overhead mainly comes from two parts. One is from the CS who sends all the encrypted distances to the verifier which contains $O(Nm/d)$ communication cost. Another one is the result from secure revealing process which requires $O(ml)$ communication. We can obtain the overall communication complexity as $O(Nm/d+ml)$. The computation overhead is more complex. We set the computation for data encryption using HE as $C_{en}$, for homomorphic multiplication as $C_{mul}$, for homomorphic addition as $C_{add}$, for key switching as $C_{sw}$, for secure comparison as $C_{com}$ and for secure~\textit{B2A} as $C_{cov}$. The overall computation overhead for the CS side is $O((Nm/d)(C_{com}+C_{add} + C_{sw}) + m(C_{com}+C_{cov}))$ and for the verifier side is $O(C_{en} + m(C_{com}+C_{cov}))$.

\subsection{Security Analysis}
% We have Theorem~\ref{theorem:security} to capture the security of CryptoMask. 

% \begin{theorem}\label{theorem:security} Algorithm~\ref{alg:distance computation} 
% and Algorithm~\ref{alg:result-revealing} securely compute the functionality $f$ in $f_{com}$-hybrid model against a semi-honest adversary.
% \end{theorem}

\textbf{Privacy of Face Vector Matrix}. 
In CryptoMask, all face vectors are encrypted by HE, and only the KG knows the secret key. Due to the semantic security of HE, neither CS or verifier learns sensitive information about the underlying encrypted face vector, thus the privacy of face vector is always maintained. 

Now we show CryptoMask only reveals a face recognition result to the verifier, and nothing else to either party. 
This is argued as regards to a corrupted CS and a corrupted verifier respectively.

\textbf{Adversarial CS.} We first demonstrate the security against a semi-honest CS. Intuitively, the security against a semi-honest CS comes from the fact that the CS's view of the execution includes only ciphertext, thus reducing the argument to semantic security of HE. We now give the formal argument. 

Let $\mathcal{A}$ be a semi-honest CS in the real protocol. We construct a simulator $\mathcal{S}$ in the ideal world as follows:

\begin{enumerate}
    \item[1.]At the beginning of the protocol execution, $\mathcal{S}$ receives the input $\boldsymbol{\mathsf{A}}$ from the environment $\mathcal{E}$ and also receives the public key $pk$ and the vector length $d$. The simulator sends $\boldsymbol{\mathsf{A}}$ to the trusted party.
    \item[2.]Start running $\mathcal{A}$ on input $\boldsymbol{\mathsf{A}}$. Next, $\mathcal{S}$ computes and sends a ciphertext $ct$ which is the encryption of a $d$ dimensional vector $\boldsymbol{0}$ to the CS under the public key $pk$.
    \item[3.]Output whatever $\mathcal{A}$ outputs.
\end{enumerate}
We argue the above simulated view is indistinguishable from real protocol execution. 
Using the fact that $\mathcal{A}$ is semi-honest, we have that at the end of the scheme in the real world, the verifier obtains $\boldsymbol{\mathsf{A}}(\boldsymbol{\mathsf{b}})$ where $\boldsymbol{\mathsf{b}}$ is the verifier's queried face image. Since $\mathcal{S}$ is semi-honest, this also holds in the ideal world. Since $\boldsymbol{\mathsf{A}}(\boldsymbol{\mathsf{b}})$ is a deterministic function, the joint distribution of the verifier's output and the adversary's output decomposes. Thus, it is suffice to show that the simulated view from $\mathcal{S}$ is computationally indistinguishable from the real view from $\mathcal{A}$.

The view of $\mathcal{A}$ in the real world contains one part: the encrypted face image ${ct}$ from the verifier. When interacting with the simulator $\mathcal{S}$, adversary $\mathcal{A}$ sees an encryption of $\boldsymbol{0}$. Security follows immediately by the semantic security of the BFV scheme.

\textbf{Adversarial Verifier.} We now prove the security against a semi-honest verifier. We construct a simulator $\mathcal{S}$ in the ideal world as follows:

\begin{enumerate}
    \item[1.]At the beginning of the execution, $\mathcal{S}$ receives the input $\boldsymbol{\mathsf{b}}$ from the environment $\mathcal{E}$ and also receives the BFV key pairs $(pk,sk)$ and the matrix size $m,d$. The simulator sends $\boldsymbol{\mathsf{b}}$ to the trusted party.
    \item[2.]Start running $\mathcal{A}$ on input $\boldsymbol{\mathsf{b}}$. Next, $\mathcal{S}$ computes and sends ciphertexts $c_i$ which is the encryption of a $m \times d$ matrix filled by some random values to the verifier under public key $pk_v$.
    \item[3.]Output whatever $\mathcal{A}$ outputs.
\end{enumerate}
In the end of face recognition, the CS has no output. Thus, to show security against a semi-honest verifier, it suffices to show that the output of $\mathcal{S}$ is computationally indistinguishable from the output of the adversary $\mathcal{A}$. Now we show the view of simulator $\mathcal{S}$ in the ideal world is computationally indistinguishable from the view of the adversary $\mathcal{A}$ in the real world.

The view of $\mathcal{A}$ in the real world contains one part: the encrypted face database $\{c_1, \cdots, c_n\}$ from CS. When interacting with the simulator $\mathcal{S}$, adversary $\mathcal{A}$ sees the encryption of random values. Security follows immediately by the semantic security of the BFV scheme.

